Fast Approximate Spectral Normalization for Robust Deep Neural Networks

Deep neural networks (DNNs) play an important role in machine learning due to its outstanding performance compared to other alternatives. However, DNNs are not suitable for safety-critical applications since DNNs can be easily fooled by well-crafted adversarial examples. One promising strategy to counter adversarial attacks is to utilize spectral normalization, which ensures that the trained model has low sensitivity towards the disturbance of input samples. Unfortunately, this strategy requires exact computation of spectral norm, which is computation intensive and impractical for large-scale networks. In this paper, we introduce an approximate algorithm for spectral normalization based on Fourier transform and layer separation. The primary contribution of our work is to effectively combine the sparsity of weight matrix and decomposability of convolution layers. Extensive experimental evaluation demonstrates that our framework is able to significantly improve both time efficiency (up to 60\%) and model robustness (61\% on average) compared with the state-of-the-art spectral normalization.

==> sections/background.tex <==
\section{Backgroudns}
\subsection{Adversarial Attack}
Even though Deep learning has earned much reputation as a powerful learning approach applied to a broad spectrum of tasks, the adversarial attack proposed by Szegedy et al.\cite{Sze2014} revealed the vulnerability of most existing neural networks against adversarial examples. 

Adversarial samples are a type of sample that is maliciously designed to attack a machine learning model. The difference between them and the original sample can hardly be distinguished by naked eyes, but will lead the model to give a false output with high confidence.
%Give an example picture
The existence of adversarial samples make the application of deep learning in fields of security seriously threatened, and how to effectively defend them is an important research topic.
\begin{figure}[htbp]
\centering
\includegraphics[scale=0.2]{sections/figs/adversarial_example.jpg}
\caption{An example of adversarial example}
\label{fig:Figure 1}
\end{figure}


Recent researchers have developed several countermeasures %cites
to defend adversarial attacks, but few of them are strong enough to tackle multiple types of attack algorithms. Spectral norm regularization proposed by Yuichi Yoshida et al.\cite{SNCNN} is one of the most appreciated approach to achieve high robustness and versatility. However, the expensive time complexity of spectral norm computation makes it difficult to get extended to deeper neural networks. For accelerating spectral norm regularization, people primarily focused on coarse approximation algorithms that sacrifices accuracy to achieve acceptable computation latency, but that is definitely harmful to the performance. One of the major contributions in this paper is to address this problem and provide a fast and dependable approximation algorithm for it.  

In next subsection, we provide prerequisite knowledge on neural networks and linear algebra based on which we can demonstrate spectral norm regularization.

\subsection{Forward Pass as Matrix Multiplication}
In this section we will illustrate how neural networks' forward pass is closely related to matrix multiplication, by which we can utilize linear algebra concepts to interpret a given model's stability. For simplicity, this section we only consider neural networks with one single layer, we will tackle multiple layer situation in the next subsection.


First, consider \textit{fully-connected layer}(FC). It is a well-known fact that each output node of FC is nothing but a weighted sum of input features as demonstrate in \textbf{Figure 2}. 
\begin{figure}[htbp]
\centering
\includegraphics[scale =0.2]{sections/figs/fig2_FC.png}
\caption{Fully Connected layer}
\label{fig:Figure 1}
\end{figure}
The bias term is ignored here because they can always be considered as another input entree with fixed weight 1. If we stack all equations up and view it as a linear system, easily we write it out in the form of matrix multiplication.
\[
\begin{bmatrix}
w_{11} & w_{12} & w_{13}\\
w_{21} & w_{22} & w_{23}\\
\end{bmatrix} \cdot
\begin{bmatrix}
a_1 \\
a_2 \\
a_3
\end{bmatrix}
= 
\begin{bmatrix}
b_1 \\
b_2 
\end{bmatrix}
\]


Now we shift our eyes to convolution neural networks, which is widely applied in computed vision and image processing tasks. \textbf{Figure 3} shows a typical example of convolution layer. A convolution kernel will sliding along the surface of input feature map and each computed weighted sum is dumped into one entree of output feature map. This matrix convolution operation is usually denoted as $`*`$.
\begin{figure}[htbp]
\centering
\includegraphics[scale =0.25]{sections/figs/fig3_CNN.png}
\caption{Convolution layer}
\label{fig:Figure 3}
\end{figure}

Assume we are dealing with a convolution layer containing only single input and single output channel, input feature map being $\textbf{A}$ and convolution kernel being $\textbf{B}$ . Then we claim 
\[
   vec(\textbf{A} * \textbf{B}) = W \cdot x
\]
where $vec(\cdot)$ is the vectorization function, $W$ is the corresponding unrolled matrix of convolution kernel $B$, which is a special case of Toeplitz matrix called doubly block circulant matrix. $x$ is simply a column vector by stretching $A$ straight.
Below we show a trivial example for better illustration of above claim. 
\[
\begin{split}
& \begin{bmatrix}
x_1 & x_2 & x_3\\
x_4 & x_5 & x_6\\
x_7 & x_8 & x_9\\
\end{bmatrix} *
\begin{bmatrix}
k_1 & k_2\\
k_3 & k_4
\end{bmatrix}\\
\overset{vec}{\Longrightarrow{}}&
\begin{bmatrix}
k_1 & k_2 & 0 & k_3 & k_4 & 0 & 0 & 0 & 0\\
0 & k_1 & k_2 & 0 & k_3 & k_4 & 0 & 0 & 0\\
0 & 0 & k_1 & k_2 & 0 & k_3 & k_4 & 0 & 0\\
0 & 0 & 0 & k_1 & k_2 & 0 & k_3 & k_4 & 0
\end{bmatrix}
\cdot
\begin{bmatrix}
x_1 \\ x_2 \\ ... \\ x_9
\end{bmatrix}\\
= & \begin{bmatrix}
k_1x_1+k_2x_2+k_3x_4+k_4x_5 \\
k_1x_2+k_2x_3+k_3x_5+k_4x_6 \\
k_1x_4+k_2x_5+k_3x_7+k_4x_8 \\
k_1x_5+k_2x_6+k_3x_8+k_4x_9
\end{bmatrix}
\end{split}
\]

 Now we come back to adversarial attacks, where most attacks are in the form of perturbing input image by tiny noise which is invisible to human eyes but these contaminated inputs can successfully fool models to spit out ill outputs. Since we have already shown the close relationship between forward pass and matrix multiplication, we can interpret adversarial attack scenarios into the language of linear algebra. Basically, assume our model's interpreted matrix (we will call this \textit{weight matrix} in the rest of this paper) is $W \in \mathbb{R}^{m \times n}$, and there is a well-crafted noise $\xi \in \mathbb{R}^{n}$ added to our input vector $x \in \mathbb{R}^{n}$, then we measure change of output by the following relative error $\epsilon \in \mathbb{R}$:
\[
\epsilon = \frac{||W \cdot (x + \xi) - W \cdot x||_2}{||\xi||_2} = \frac{||W \cdot \xi||_2}{||\xi||_2}
\]
This is input-irrelevant, and recall the spectral norm $\sigma(W)$ of matrix $W$ is defined as:
\[
\sigma(W) = \max \limits_{\xi \neq \textbf{0}}\frac{||W\cdot \xi||_2}{||\xi||_2}
\]
Therefore, spectral norm of matrix $W$ gives a tight upperbound of given layer's stability, and a small value of $\sigma(W)$ indicates this model's insensitivity to the perturbation of input $x$. Consequently, if we append the spectral norm of $W$ to loss function as a penalty term, we hopefully will obtain a more stable model which becomes resistant towards adversarial attacks.\\

\subsection{Spectral Norm Regularization}
In actual applications we always have to face up with models containing multiple layers and activation layers, so in this section we explain how the spectral norm is actually utilized in network training as a regularizer.\\
% 1. Activation layers
% 2. Squeeze cascaded as a sequantial multiplication, and it suffices to bound the summation.
% 3. modified loss function
% 4. algorithm
% 5. compared with other regularizers(just say sth with references) Hence, we exclude these regularizations from our experiments and focus on the comparison between Yuichi Yoshida's original post and our refined approach.
\textbf{Activation Functions.} Activation functions are inserted between consecutive network layers to induce nonlinearity, because nonlinearity allows deep neural networks to complete nontrivial tasks with limited number of nodes. But nowadays, activation functions are usually selected as piecewise linear functions, such as ReLU , maxout [10], and maxpooling [26]. If that is the case, since adversarial examples always reside in the close neighborhood of given input, we can still consider activation function as a linear function, or more precisely, an affine map under adversarial attack scenarios. Affine maps are absolutely compatible with matrix representation. \\
\textbf{Multiple Layers.} Once we tackle activation functions between consecutive layers, we are able to represent the forward pass of multiple layers as a \textit{cascaded matrix multiplication}. Explicitly, assume a model contains $K$ layers and $W^k$ denotes the weight matrix of the $k$-th layer where $k\in\{1,...,K\}$. Then by similar derivation process in previous section, the stability of given model is bounded by $\prod \limits_{k=1}^K \sigma(W^k)$. \\
\textbf{Modified Loss Function.} For general neural network, given training dataset, the loss function $J$ is usually defined as: 
\[ J = \frac{1}{N}\sum \limits_{i=1}^{N} L(f(x_i), y_i)\]
Here, $x_i$ is a training sample, the label of $x_i$ is denoted as $y_i$, and the total number of training samples in a batch is denoted as $N$, $L$ is the dissimilarity measurement and is frequently selected to be cross entropy or squared $l_2$ distance. We'd like to append our spectral norm product $\prod \limits_{k=1}^K \sigma(W^k)$ as a penalty term to this loss function. Notice that $\sigma(W^k) \geq 0$ holds for any matrix, so it suffices to bound the spectral norm of each $W^k$. Therefore, for computational convenience we append the squared summation of spectral norms instead of their product to obtain the modified loss function as follows:
\[ J = \frac{1}{N}\sum \limits_{i=1}^{N} L(f(x_i), y_i) + \frac{\lambda}{2}\sum\limits_{k=1}^K\sigma(W^k)^2 \]
Here $\lambda \in \mathbb{R}^+$ is a regularization factor.
\\
\textbf{Modified SGD.} A widely used idea to train a neural network is \textit{stochastic gradient descent}(SGD). When performing SGD for our modified loss function, we need to calculate the gradient of $\frac{\lambda}{2}\sum\limits_{k=1}^K\sigma(W^k)^2$, which can be approached as $\lambda\sum\limits_{k=1}^K\sigma_{k}\textbf{u}_{k}\textbf{v}^{\top}_{k}$ illustrated in~\cite{SNCNN}, where $\sigma_{k}$ is the largest singular value of $k$-th weight matrix $W^k$, $\textbf{u}_{k}$ and $\textbf{v}_{k}$ are the corresponding left and right singular vectors. The baseline method in~\cite{SNCNN} applied power iteration to approximate $\sigma_{k}$, $\textbf{u}_{k}$ and $\textbf{v}_{k}$, this algorithm is demonstrated as pseudocode shown in \textbf{Algorithm1}.

\begin{algorithm}
    \caption{SGD with spectral norm regularization}
    \begin{algorithmic}[1] % show lines 
        \For {each iteration of SGD}
            \State Compute the gradient of general loss function as usual
            \For {$k = 1$ to $K$}
            \State $\textbf{v}_k \leftarrow$ random gaussian vector
                \For {a sufficient number of times}
                    \State $\textbf{u}_k \leftarrow W^k\textbf{v}_k$
                    \State $\textbf{v}_k \leftarrow (W^k)^\top \textbf{u}_k$
                    \State $\sigma_k \leftarrow ||\textbf{u}_k||_2 / ||\textbf{v}_k||_2$
                \EndFor
                \State Add $\lambda\sigma_k\textbf{u}_k\textbf{v}_k $ to gradient
            \EndFor
            \State Update parameters using modified gradient
        \EndFor
    \end{algorithmic}
\end{algorithm}




==> sections/case.tex <==
\section{Experiments}
\label{exp}
We evaluated the effectiveness of our optimized spectral norm regularization framework to confirm its time efficiency and ability of enhancing DNNs' robustness.

\subsection{Experimental Setup}
Experiments are conducted on a host machine with Intel i7 3.70GHz CPU, 32 GB RAM and RTX 2080 256-bit GPU. We developed code using Python for model training. We used PyTorch as the machine learning library. For adversarial attack algorithms, we utilized the \textit{Adversarial Robustness 360 Toolbox} (ART)~\cite{art2018}. Based on this environment, we considered the following two settings for our experimental evaluation:

% We implement our RFB Net detector based on the framework of Pytorch
% , utilizing several parts of open source infrastructures provided by the ssd.pytorch
% repository2
% . Our training strategies mostly follow SSD, including data augmentation, hard negative mining, scale and aspect ratios for default boxes, and loss
% functions (e.g., smooth L1 loss for localization and softmax loss for classification),
% while we slightly change our learning rate scheduling for better accommodation
% of RFB. More details are given in the following section of experiments. All new
% conv-layers are initialized with the MSRA method
\begin{enumerate}
    \item The AlexNet~\cite{Alexnet} neural network for MNIST~\cite{MNIST} dataset.
    \item The VGG19~\cite{VGG19} for ImageNet~\cite{imagenet} dataset.
\end{enumerate}
For each setting we compare the following three approaches:
%\begin{enumerate}
\textbf{Normal}: Ordinary training without general $L$-2 regularization~\cite{L2}, which is considered as control group.\\
\textbf{SN}: State-of-the-art approach (Algorithm~\ref{Alg1}) with spectral normalization~\cite{SNCNN}.\\
\textbf{FSN}: Our proposed approach (Algorithm~\ref{Alg3}) with fast spectral normalization.
%\end{enumerate}

As for result evaluation, we first evaluated the functionality of them by reporting their accuracy and training time. Next, both bounded and unbounded adversarial attacks were deployed to test their robustness. We applied the following four adversarial attack algorithms: FGSM~\cite{FSGM}, DeepFool~\cite{DeepFool}, JSMA~\cite{JSMA} and PGD~\cite{CarliniW16a}.
\begin{enumerate}
    \item FGSM: A gradient based lightweight attack algorithm. Usually applied for sanity check.
    \item DeepFool: An untargeted attack technique optimized for the $L$2 distance metric. 
    \item JSMA:  A Jacobian-based Saliency Map attack implemented by saturating pixels of input image.
    \item PGD: Projected gradient descent based attack. It is among the strongest attacks utilizing the local first order information about the network.
\end{enumerate}

We tuned the regularizer factor $\lambda$ for FSN to demonstrate its stability across a wide variety of different $\lambda$ values. 

%\vspace{-0.2in}
\subsection{Case Study: MNIST benchmark}
We train AlexNet on MNIST dataset. AlexNet contains 5 convolutional Layers and 3 Fully Connected Layers. 
% One advantage of AlexNet is the replacement of larger convolution kernels ($11\times11, 7\times7, 5\times5$) with consecutive $3\times3$ convolution kernels, which makes it coincidentally suitable for our framework since small size of convolution kernel implies less time cost for low-rank approximation.
We choose a mini-batch size of 64. For each setting, we train the network with 200 epochs. For every 10 epochs, we randomly shuffle and split $80\%$ as training set and $20\%$ as test set, and then report the training time along with test performance.

\begin{table}[htbp]
    \caption{Training time and test accuracy of AlexNet}
    %\vspace{20pt}
    \centering
    \begin{tabular}{c|cc}
        \hline
        \thead[l]{Methods} & \thead[l]{Time(s/epoch)}& \thead[l]{Best Test Accuracy(\%)} \\
        \hline
        Normal  & 14.5053   & 83.45 \\
        SN  & 29.1126   & 91.72 \\
        FSN & 18.1345   & 95.46 \\
        \hline       
    \end{tabular}
    \label{Tb1}
\end{table}

Table~\ref{Tb1} indicates the basic functionality performance of three training methods. We also plot the training curve for accuracy updates in Figure~\ref{fig:label6}. In general, all three methods possess good training accuracy. The Normal approach achieved the fastest speed but when it comes to test accuracy, it lagged behind the other two due to spectral normalization's ability to enhance model's generalizability~\cite{SNCNN}. SN promote the test accuracy by $8.27\%$ but also introduces the highest time cost due to the slow converging speed of power iteration. FSN further improves the test accuracy by $3.66\%$ while reduces average training time by $37.9\%$ compared with SN.

Table~\ref{Tb2} shows the performance of three models against bounded attacks. For consistency, we use $\lambda = 0.01$ for both SN and FSN here. The hyperparameters for attacks are provided in the table.

\vspace{-0.1in}
\begin{figure}[htbp]
\centering
\includegraphics[scale =0.2]{sections/figs/GTSB_basic.png}
\vspace{-0.05in}
\caption{Accuracy curve of AlexNet on MNIST}
\label{fig:label6}
\end{figure}
%\vspace{-0.1in}



%\vspace{-0.05in}
\begin{table}[tp]
    \caption{Bounded attack on MNIST}
    %\vspace{20pt}
    \centering
    \begin{tabular}{c|ccccc}
        \hline
        \thead[l]{Methods} & \thead[l]{N/A}& \thead[l]{FGSM \\($\varepsilon$ = .1)} & \thead[l]{$\,\,\,$DeepFool\\($\varepsilon=1e-6$)} & \thead[l]{$\quad\,\,$JSMA \\$(\theta,\gamma = .1,1)$} & \thead[l]{$\,\,\,$PGD\\ ($\varepsilon=0.3$)}\\
        \hline
        Normal   & 83.45 & 61.04 & 45.62 & 77.58 & 40.06 \\
        SN   & 91.72 & 88.25 & 76.31 & 88.23 & 69.30\\
        FSN & 95.46 & 92.92 & 87.05 & 91.57 & 88.94 \\
        \hline       
    \end{tabular}
    \label{Tb2}
    \\\vspace{-0.15in}
\end{table}
As we can see, our proposed method (FSN) provides the best robustness. The Normal and SN method appear fragile in the face of powerful attacks like DeepFool and PGD, while FSN still retained an acceptable accuracy. For lightweight attacks, especially gradient-based ones (like FGSM), FSN is almost unaffected. For unbounded attack, we applied unbounded incremental $\varepsilon$ value in FGSM from 0 to 1. It starts to break detection (accuracy $<$ 50\%) as presented in Figure~\ref{fig:label7}(a), but the bisection parameter value of FSN($\varepsilon= .64$) has to be nearly three times large of that for Normal method ($\varepsilon= .21$). Finally, FSN's  robust performance across a wide range of hyperparameter $\lambda$ is demonstrated in Figure~\ref{fig:label7}(b) where we plot accuracy under all attacks with $\lambda$ varying from 0.01 to 0.1. The average accuracy here is $91.46\%$ with standard deviation of 0.0729. In the worst case, model trained with FSN still performed well with accuracy above $85\%$.

%\vspace{-0.2in}
\begin{figure}[htbp]
\centering
\subfigure[Performance of three models towards unbounded FGSM attack] {\includegraphics[height=1.3in,width=1.6in]{sections/figs/unbounded.png}}
\subfigure[FSN's performance with different $\lambda$ and attack algorithm] {\includegraphics[height=1.3in,width=1.6in]{sections/figs/lambda1.png}}
\vspace{-0.1in}
\caption{Performance with varying hyperparameter (MNIST)}
\label{fig:label7}
\end{figure}
\vspace{-0.1in}

\subsection{Case Study: ImageNet benchmark}
We trained VGG19 on ImageNet. Compared with AlexNet, VGG19 is a deeper network. It is a variant of VGG model consisting of 19 layers (16 convolution layers, 3 fully connected layer, 5 maxpool layers and 1 softmax layer). One advantage of VGG19 is the replacement of larger convolution kernels ($11\times11, 7\times7, 5\times5$) with consecutive $3\times3$ convolution kernels, which makes it coincidentally suitable for our framework since small size of convolution kernel implies less time cost for low-rank approximation. The training process consists of 500 epochs with a mini-batch size of 128. For every 50 epochs, we randomly shuffle sample and split $80\%$ as training set and $20\%$ as test.

\begin{table}[htbp]
    \caption{Training time and test accuracy of VGG19}
    %\vspace{20pt}
    \centering
    \begin{tabular}{c|cc}
        \hline
        \thead[l]{Methods} & \thead[l]{Time(s/epoch)}& \thead[l]{Best Test Accuracy(\%)} \\
        \hline
        Normal  & 23.969   & 99.71 \\
        SN      & 121.886   & 98.57 \\
        FSN     & 49.037   & 99.43 \\
        \hline       
    \end{tabular}
    \label{Tb3}
\end{table}

Table~\ref{Tb3} and Figure~\ref{fig:label8} present performance results. Again, Normal method provides the fastest training speed, while FSN is nearly $60.4\%$ faster than SN. Note that the improvement of speed here is even better than we got from MNIST case, and we consider this difference of acceleration amplitude is caused by more convolution layers involved along with smaller size of kernels. For accuracy, due to VGG19's excellent capability in image recognition, all three models achieved high level of accuracy.

\begin{figure}[h]
\vspace{-0.2in}
\centering
\includegraphics[scale=0.19]{sections/figs/USD_basic.png}
\vspace{-0.1in}
\caption{Accuracy curve of VGG19 on ImageNet}
\label{fig:label8} 
\vspace{-0.1in}
\end{figure}

 The robustness is evaluated against four attack algorithms as shown in Table~\ref{Tb4}. As expected, Normal method behaved extremely vulnerable. Even in $\varepsilon = 0.1$ case, a $8.3\%$ accuracy against FGSM attack was obtained. FSN refined it to $71.4\%$ which gives an 61.1\% average improvement on accuracy. When it comes to unbounded attack as depicted in Figure~\ref{fig:label9}(a), the Normal method's outcome immediately drops below $50\%$ when $\varepsilon = 0.1$, while SN and FSN extended it to $0.4$ and $0.5$, respectively. Figure~\ref{fig:label9}(b) shows the accuracy after applying various regularization factor of $\lambda$. The average accuracy is 62.63\% with standard deviation of 0.2252. In the worst case, model trained with FSN  still performed well with accuracy near 70\% by setting regularization factor $\lambda = 0.1$.
 
 
 \begin{table}[H]
    \caption{Bounded attack on ImageNet}
    %\vspace{20pt}
    \centering
    \begin{tabular}{c|ccccc}
        \hline
        \thead[l]{Methods} & \thead[l]{N/A}& \thead[l]{FGSM \\($\varepsilon$ = .1)} & \thead[l]{$\,$DeepFool\\($\varepsilon$=1e-6)} & \thead[l]{$\,\,$JSMA \\$(\theta,\gamma = .1,1)$} & \thead[l]{$\,\,$PGD\\ ($\varepsilon=0.3$)}\\
        \hline
        Normal   & 99.71 & 8.3 & 5.62 & 17.58 & 4.06 \\
        SN       & 98.57 & 69.9 & 34.34 & 78.23 & 29.30\\
        FSN      & 99.43 & 71.4 & 70.05 & 82.34 & 68.94 \\
        \hline       
    \end{tabular}
    \label{Tb4}
\end{table}

 
\begin{figure}[htbp]
\centering
\subfigure[Performance of three models under unbounded FGSM attack] {\includegraphics[width=1.72in]{sections/figs/unbounded_USD.png}}
\subfigure[FSN's performance with different $\lambda$ and attack algorithm] {\includegraphics[width=1.72in]{sections/figs/lambda2.png}}
%\vspace{-0.1in}
\caption{Performance with varying hyperparameters (ImageNet)}
%\vspace{-0.1in}
\label{fig:label9}
\end{figure}
